Universal family of the subgroups of an algebraic group

We construct a moduli space for the connected subgroups of an algebraic group and the corresponding universal family. Morphisms from an algebraic variety to this moduli space correspond to flat families of connected algebraic subgroups parametrised by this variety. This moduli space is obtained by gluing together infinitely many irreducible projective varieties of bounded dimension along closed subvarieties. Regarding families of non-connected subgroups of an algebraic group, we show that, given sich a family, the corresponding family of identity components is an irreducible component of the former, and the quotient of a family of groups group by the family of their identity components exists.

==> alglie.tex <==
\section{Algebraic Lie algebras}


==> appga.tex <==
\section{Results of algebraic geometry}

\begin{proposition}
\label{pr:ag:ncirr}
Let~$X$ and~$P$ be projective varieties and let~$\mathcal{F}$ be a family of
subvarieties of~$X$ parametrized by~$P$. The number of irreducible components
in a fiber of~$\mathcal{F}$ has a uniform bound on~$P$.
\end{proposition}

\begin{proof}
The projective morphism~$\mathcal{F}\to P$ decomposes into a Veronese
embedding followed by a linear projection, hence we can assume
that~$\mathcal{F}$ is a subvariety of a projective space~$\P(E)$, that~$P$
is a linear subspace of~$\P(E)$, and that~$\mathcal{F}\to P$ is a linear
projection. By induction on the dimension of~$P$, we only need to show that
the number of irreducible components in a hyperplane
section~$\mathcal{F} \cap H$ of~$\mathcal{F}$ has a bound independant
of~$H$. The degree of~$\mathcal{F}$ is such a bound.
\end{proof}

% Local Variables:
% ispell-dictionary: "en"
% End:

